Radioactive nuclei in the early Solar System: analysis of the 15 isotopes produced by core-collapse supernovae

Short-lived radioactive isotopes (SLRs) with half-lives between 0.1 to 100 Myr can be used to probe the origin of the Solar System. In this work, we examine the core-collapse supernovae production of the 15 SLRs produced: $^{26}$Al, $^{36}$Cl, $^{41}$Ca, $^{53}$Mn, $^{60}$Fe, $^{92}$Nb, $^{97}$Tc, $^{98}$Tc, $^{107}$Pd, $^{126}$Sn, $^{129}$I, $^{135}$Cs, $^{146}$Sm, $^{182}$Hf, and $^{205}$Pb. We probe the impact of the uncertainties of the core-collapse explosion mechanism by examining a collection of 62 core-collapse models with initial masses of 15, 20, and 25M$_{\odot}$, explosion energies between 3.4$\times$10$^{50}$ and 1.8$\times$10$^{52}$ ergs and compact remnant masses between 1.5M$_{\odot}$and 4.89M$_{\odot}$. We identify the impact of both explosion energy and remnant mass on the final yields of the SLRs. Isotopes produced within the innermost regions of the star, such as $^{92}$Nb and $^{97}$Tc, are the most affected by the remnant mass, $^{92}$Nb varying by five orders of magnitude. Isotopes synthesised primarily in explosive C-burning and explosive He-burning, such as $^{60}$Fe, are most affected by explosion energies. $^{60}$Fe increases by two orders of magnitude from the lowest to the highest explosion energy in the 15M$_{\odot}$model. The final yield of each examined SLR is used to compare to literature models.

==> tables/Summary_data_table1.tex <==
\begin{table*}
\centering
\begin{tabular}{rrrr|rrrrrr}
M$_{prog}$& E$_{exp}$& M$_{rem}$& Dilution ($f$) & $^{36}$Cl & $^{41}$Ca & $^{53}$Mn & $^{60}$Fe & $^{92}$Nb & $^{107}$Pd \\ 
(M$_{\odot})$ & FoE & (M$_{\odot})$ &  &  &  &  &  &  &  \\ 
\hline
15 & 1.90 & 1.62  & 1.600$\times$10$^{-4}$ & 0.16 & 1.85 & 41.8 & 348.24 & 286.6 & 9.69 \\ 
15 & 1.86 & 1.63  & 1.598$\times$10$^{-4}$ & 0.16 & 1.84 & 41.98 & 339.03 & 326.47 & 9.82 \\ 
15 & 1.94 & 1.61  & 1.601$\times$10$^{-4}$ & 0.16 & 1.87 & 41.95 & 354.77 & 269.35 & 9.64 \\ 
15 & 0.54 & 1.91  & 1.484$\times$10$^{-4}$ & 0.14 & 0.55 & 0.89 & 284.73 & 0.01 & 10.98 \\ 
15 & 0.92 & 1.75  & 1.617$\times$10$^{-4}$ & 0.19 & 1.35 & 20.59 & 340.8 & 73.27 & 9.94 \\ 
15 & 1.69 & 1.52  & 1.561$\times$10$^{-4}$ & 0.15 & 1.79 & 47.55 & 351.85 & 4198.28 & 9.33 \\ 
15 & 0.34 & 1.94  & 1.448$\times$10$^{-4}$ & 0.13 & 0.42 & 0.65 & 278.83 & 0.01 & 10.87 \\ 
15 & 3.43 & 1.51  & 1.676$\times$10$^{-4}$ & 0.19 & 1.75 & 42.57 & 1357.03 & 3046.72 & 8.36 \\ 
15 & 2.06 & 1.59  & 1.603$\times$10$^{-4}$ & 0.16 & 1.89 & 45.96 & 369.03 & 1890.73 & 9.52 \\ 
15 & 2.24 & 1.56  & 1.605$\times$10$^{-4}$ & 0.16 & 1.9 & 50.85 & 408.17 & 6603.52 & 9.34 \\ 
15 & 2.60 & 1.52  & 1.601$\times$10$^{-4}$ & 0.15 & 1.86 & 49.44 & 559.39 & 7089.44 & 8.93 \\ 
15 & 0.74 & 1.73  & 1.637$\times$10$^{-4}$ & 0.19 & 1.36 & 15.17 & 336.11 & 63.19 & 10.36 \\ 
15 & 0.82 & 1.88  & 1.522$\times$10$^{-4}$ & 0.15 & 1.23 & 7.52 & 294.2 & 0.01 & 10.84 \\ 
15 & 10.7 & 1.53  & 1.922$\times$10$^{-4}$ & 0.21 & 2.55 & 38.16 & 376.94 & 2500.34 & 11.41 \\ 
15 & 2.47 & 1.52  & 1.725$\times$10$^{-4}$ & 0.17 & 1.93 & 40.82 & 403.84 & 346.31 & 9.97 \\ 
15 & 4.79 & 1.50  & 1.810$\times$10$^{-4}$ & 0.22 & 1.85 & 37.73 & 2333.93 & 3105.44 & 7.85 \\ 
15 & 2.63 & 1.53  & 1.820$\times$10$^{-4}$ & 0.2 & 2.14 & 49.91 & 878.52 & 3252.31 & 9.45 \\ 
20 & 2.85 & 1.74  & 6.050$\times$10$^{-4}$ & 7.28 & 11.33 & 2406.52 & 822.19 & 0.02 & 135.48 \\ 
20 & 1.47 & 2.23  & 6.618$\times$10$^{-4}$ & 0.44 & 3.86 & 366.43 & 879.76 & 0.0 & 145.96 \\ 
20 & 2.50 & 1.93  & 4.711$\times$10$^{-4}$ & 5.95 & 3.64 & 20.1 & 658.71 & 0.02 & 103.54 \\ 
20 & 5.03 & 1.74  & 3.743$\times$10$^{-4}$ & 1.41 & 8.34 & 1381.89 & 719.13 & 58.33 & 74.89 \\ 
20 & 2.76 & 1.76  & 5.854$\times$10$^{-4}$ & 7.58 & 11.22 & 2368.72 & 804.2 & 0.02 & 130.46 \\ 
20 & 2.60 & 1.90  & 5.627$\times$10$^{-4}$ & 7.41 & 9.38 & 265.57 & 792.45 & 0.02 & 124.84 \\ 
20 & 2.43 & 1.86  & 5.998$\times$10$^{-4}$ & 7.19 & 10.46 & 1396.44 & 814.98 & 0.02 & 134.26 \\ 
20 & 1.04 & 2.47  & 7.038$\times$10$^{-4}$ & 0.44 & 3.75 & 373.82 & 822.63 & 0.0 & 142.37 \\ 
20 & 4.15 & 1.85  & 3.749$\times$10$^{-4}$ & 1.41 & 7.87 & 1392.13 & 689.3 & 0.11 & 77.32 \\ 
20 & 0.65 & 3.03  & 7.062$\times$10$^{-4}$ & 0.45 & 3.14 & 2.15 & 577.46 & 0.0 & 112.47 \\ 
20 & 0.78 & 2.85  & 7.056$\times$10$^{-4}$ & 0.39 & 3.33 & 250.74 & 654.81 & 0.0 & 122.13 \\ 
20 & 0.84 & 2.62  & 7.048$\times$10$^{-4}$ & 0.42 & 3.58 & 316.56 & 755.27 & 0.0 & 134.4 \\ 
20 & 1.00 & 2.35  & 7.023$\times$10$^{-4}$ & 0.45 & 3.88 & 400.72 & 875.39 & 0.0 & 148.53 \\ 
20 & 1.65 & 1.78  & 6.711$\times$10$^{-4}$ & 5.58 & 10.34 & 1600.17 & 908.89 & 0.01 & 151.37 \\ 
20 & 0.75 & 2.76  & 7.053$\times$10$^{-4}$ & 0.4 & 3.43 & 303.65 & 693.74 & 0.0 & 126.94 \\ 
20 & 0.53 & 3.40  & 7.076$\times$10$^{-4}$ & 0.34 & 2.74 & 0.04 & 418.51 & 0.0 & 92.6 \\ 
20 & 4.33 & 1.87  & 3.680$\times$10$^{-4}$ & 1.26 & 7.79 & 1537.8 & 687.62 & 0.12 & 74.39 \\ 
20 & 0.81 & 2.70  & 7.051$\times$10$^{-4}$ & 0.41 & 3.5 & 331.27 & 720.73 & 0.0 & 130.22 \\ 
20 & 1.19 & 2.28  & 7.000$\times$10$^{-4}$ & 0.46 & 3.96 & 385.96 & 904.97 & 0.0 & 151.8 \\ 
20 & 1.52 & 1.97  & 6.668$\times$10$^{-4}$ & 5.2 & 4.76 & 57.43 & 902.76 & 0.02 & 150.31 \\ 
20 & 1.39 & 1.93  & 6.703$\times$10$^{-4}$ & 4.88 & 4.97 & 8.91 & 907.71 & 0.01 & 151.2 \\ 
20 & 8.86 & 1.74  & 3.555$\times$10$^{-4}$ & 0.9 & 10.04 & 1581.1 & 2276.56 & 2164.45 & 57.06 \\ 
20 & 0.85 & 2.62  & 7.048$\times$10$^{-4}$ & 0.42 & 3.58 & 330.46 & 755.72 & 0.0 & 134.43 \\ 
25 & 1.92 & 3.13  & 1.051$\times$10$^{-4}$ & 1.04 & 4.26 & 699.28 & 850.91 & 0.21 & 28.3 \\ 
25 & 3.07 & 1.83  & 1.051$\times$10$^{-4}$ & 1.04 & 4.26 & 699.38 & 853.05 & 41.29 & 150244.21 \\ 
25 & 3.30 & 2.35  & 1.059$\times$10$^{-4}$ & 1.05 & 4.03 & 327.93 & 830.19 & 0.21 & 28.51 \\ 
25 & 1.04 & 1.84  & 1.333$\times$10$^{-4}$ & 1.44 & 5.67 & 571.64 & 796.35 & 41.45 & 45.08 \\ 
25 & 9.73 & 2.35  & 1.071$\times$10$^{-4}$ & 1.01 & 3.93 & 40.35 & 1407.67 & 0.21 & 24.73 \\ 
25 & 1.20 & 1.84  & 1.333$\times$10$^{-4}$ & 1.44 & 5.67 & 711.25 & 796.35 & 39.4 & 46.79 \\ 
25 & 7.42 & 2.37  & 8.412$\times$10$^{-5}$ & 0.3 & 3.67 & 443.54 & 1271.94 & 0.07 & 18.76 \\ 
25 & 18.4 & 2.35  & 1.055$\times$10$^{-4}$ & 1.0 & 3.83 & 39.09 & 1941.84 & 0.21 & 23.65 \\ 
25 & 14.8 & 2.35  & 7.676$\times$10$^{-5}$ & 0.73 & 3.92 & 399.91 & 2136.01 & 0.3 & 10.2 \\ 
25 & 2.78 & 2.35  & 1.059$\times$10$^{-4}$ & 1.05 & 4.03 & 327.96 & 830.17 & 0.21 & 28.98 \\ 
25 & 0.89 & 4.66  & 7.431$\times$10$^{-4}$ & 0.56 & 3.86 & 0.05 & 2832.12 & 0.0 & 179.17 \\ 
25 & 7.08 & 2.35  & 1.059$\times$10$^{-4}$ & 1.06 & 4.03 & 328.06 & 830.52 & 0.21 & 28.39 \\ 
25 & 0.92 & 1.84  & 1.333$\times$10$^{-4}$ & 1.44 & 5.67 & 711.25 & 796.35 & 39.39 & 47.08 \\ 
25 & 2.64 & 2.35  & 1.059$\times$10$^{-4}$ & 1.05 & 4.03 & 327.97 & 830.17 & 0.21 & 28.95 \\ 
25 & 6.17 & 2.38  & 9.114$\times$10$^{-5}$ & 0.32 & 3.96 & 474.53 & 1180.58 & 0.08 & 20.99 \\ 
25 & 4.73 & 2.38  & 1.732$\times$10$^{-4}$ & 0.49 & 6.24 & 668.74 & 1392.02 & 0.81 & 51.75 \\ 
25 & 1.52 & 1.83  & 1.333$\times$10$^{-4}$ & 1.44 & 5.67 & 711.25 & 796.35 & 39.4 & 46.79 \\ 
25 & 1.57 & 3.73  & 5.518$\times$10$^{-4}$ & 0.39 & 3.61 & 0.05 & 2427.45 & 0.0 & 175.22 \\ 
25 & 0.99 & 4.89  & 7.447$\times$10$^{-4}$ & 0.52 & 3.66 & 0.04 & 2827.98 & 0.0 & 161.83 \\ 
25 & 8.40 & 2.38  & 1.074$\times$10$^{-4}$ & 1.01 & 3.37 & 16.25 & 1452.99 & 0.22 & 24.81 \\ 
25 & 2.53 & 2.35  & 1.059$\times$10$^{-4}$ & 1.05 & 4.03 & 327.98 & 830.17 & 0.21 & 28.92 \\ 
25 & 4.72 & 2.35  & 1.059$\times$10$^{-4}$ & 1.05 & 4.03 & 327.97 & 830.3 & 0.21 & 28.38 \\ 
\end{tabular}
\label{full_summary_table:one}
\caption{Table of all core collapse model predicted/ESS ratios using $^{26}$Al as the dilution isotope. M$_{prog}$ is the progenitor mass, E$_{exp}$ is the explosion energy, M$_{rem}$ is the remnant mass.}
\end{table*}

==> tables/Summary_data_table2.tex <==
\begin{table*}
\centering
\begin{tabular}{rrrr|rrrrrr}
M$_{prog}$& E$_{exp}$& M$_{rem}$& Dilution ($f$) & $^{126}$Sn & $^{129}$I & $^{135}$Cs & $^{146}$Sm & $^{182}$Hf & $^{205}$Pb \\ 
(M$_{\odot})$ & FoE & (M$_{\odot})$ &  &  &  &  &  &  &  \\ 
\hline
15 & 1.90 & 1.62  & 1.600$\times$10$^{-4}$ & 0.47 & 0.35 & 69.78 & 0.01 & 1.66 & 14.51 \\ 
15 & 1.86 & 1.63  & 1.598$\times$10$^{-4}$ & 0.36 & 0.35 & 70.98 & 0.01 & 1.81 & 14.76 \\ 
15 & 1.94 & 1.61  & 1.601$\times$10$^{-4}$ & 0.55 & 0.35 & 69.29 & 0.01 & 1.58 & 14.38 \\ 
15 & 0.54 & 1.91  & 1.484$\times$10$^{-4}$ & 0.04 & 0.35 & 78.13 & 0.01 & 0.51 & 16.42 \\ 
15 & 0.92 & 1.75  & 1.617$\times$10$^{-4}$ & 0.23 & 0.33 & 73.71 & 0.01 & 1.95 & 15.32 \\ 
15 & 1.69 & 1.52  & 1.561$\times$10$^{-4}$ & 0.51 & 0.34 & 67.94 & 0.01 & 1.51 & 14.1 \\ 
15 & 0.34 & 1.94  & 1.448$\times$10$^{-4}$ & 0.04 & 0.33 & 74.52 & 0.0 & 0.3 & 16.29 \\ 
15 & 3.43 & 1.51  & 1.676$\times$10$^{-4}$ & 16.19 & 0.33 & 65.49 & 0.01 & 2.46 & 12.38 \\ 
15 & 2.06 & 1.59  & 1.603$\times$10$^{-4}$ & 0.73 & 0.35 & 68.48 & 0.01 & 1.43 & 14.13 \\ 
15 & 2.24 & 1.56  & 1.605$\times$10$^{-4}$ & 1.18 & 0.35 & 67.4 & 0.01 & 1.16 & 13.72 \\ 
15 & 2.60 & 1.52  & 1.601$\times$10$^{-4}$ & 3.07 & 0.34 & 66.27 & 0.01 & 1.51 & 13.03 \\ 
15 & 0.74 & 1.73  & 1.637$\times$10$^{-4}$ & 0.16 & 0.34 & 76.79 & 0.01 & 1.92 & 15.81 \\ 
15 & 0.82 & 1.88  & 1.522$\times$10$^{-4}$ & 0.05 & 0.36 & 80.64 & 0.01 & 1.09 & 16.23 \\ 
15 & 10.7 & 1.53  & 1.922$\times$10$^{-4}$ & 0.41 & 0.36 & 75.81 & 0.01 & 2.02 & 16.64 \\ 
15 & 2.47 & 1.52  & 1.725$\times$10$^{-4}$ & 1.02 & 0.35 & 69.84 & 0.01 & 1.31 & 14.55 \\ 
15 & 4.79 & 1.50  & 1.810$\times$10$^{-4}$ & 36.56 & 0.3 & 62.94 & 0.01 & 2.51 & 11.78 \\ 
15 & 2.63 & 1.53  & 1.820$\times$10$^{-4}$ & 7.56 & 0.35 & 69.38 & 0.01 & 2.22 & 13.61 \\ 
20 & 2.85 & 1.74  & 6.050$\times$10$^{-4}$ & 0.02 & 2.61 & 512.98 & 0.01 & 7.3 & 278.57 \\ 
20 & 1.47 & 2.23  & 6.618$\times$10$^{-4}$ & 0.02 & 2.55 & 528.74 & 0.0 & 7.56 & 298.86 \\ 
20 & 2.50 & 1.93  & 4.711$\times$10$^{-4}$ & 0.02 & 2.12 & 404.52 & 0.01 & 5.14 & 214.88 \\ 
20 & 5.03 & 1.74  & 3.743$\times$10$^{-4}$ & 0.81 & 1.78 & 346.98 & 0.03 & 11.62 & 160.05 \\ 
20 & 2.76 & 1.76  & 5.854$\times$10$^{-4}$ & 0.02 & 2.5 & 493.19 & 0.01 & 7.0 & 268.61 \\ 
20 & 2.60 & 1.90  & 5.627$\times$10$^{-4}$ & 0.03 & 2.39 & 471.1 & 0.01 & 6.68 & 257.13 \\ 
20 & 2.43 & 1.86  & 5.998$\times$10$^{-4}$ & 0.02 & 2.52 & 502.75 & 0.01 & 7.12 & 276.2 \\ 
20 & 1.04 & 2.47  & 7.038$\times$10$^{-4}$ & 0.02 & 2.37 & 499.97 & 0.0 & 7.12 & 286.57 \\ 
20 & 4.15 & 1.85  & 3.749$\times$10$^{-4}$ & 0.5 & 1.83 & 350.06 & 0.03 & 8.65 & 162.61 \\ 
20 & 0.65 & 3.03  & 7.062$\times$10$^{-4}$ & 0.01 & 1.57 & 355.73 & 0.0 & 4.71 & 214.28 \\ 
20 & 0.78 & 2.85  & 7.056$\times$10$^{-4}$ & 0.01 & 1.83 & 402.24 & 0.0 & 5.48 & 237.61 \\ 
20 & 0.84 & 2.62  & 7.048$\times$10$^{-4}$ & 0.02 & 2.16 & 461.37 & 0.0 & 6.47 & 267.26 \\ 
20 & 1.00 & 2.35  & 7.023$\times$10$^{-4}$ & 0.02 & 2.54 & 529.94 & 0.0 & 7.62 & 301.56 \\ 
20 & 1.65 & 1.78  & 6.711$\times$10$^{-4}$ & 0.02 & 2.69 & 554.15 & 0.01 & 8.01 & 311.5 \\ 
20 & 0.75 & 2.76  & 7.053$\times$10$^{-4}$ & 0.01 & 1.96 & 425.44 & 0.0 & 5.87 & 249.24 \\ 
20 & 0.53 & 3.40  & 7.076$\times$10$^{-4}$ & 0.01 & 1.04 & 259.91 & 0.0 & 3.11 & 166.23 \\ 
20 & 4.33 & 1.87  & 3.680$\times$10$^{-4}$ & 0.61 & 1.77 & 341.55 & 0.03 & 9.65 & 157.4 \\ 
20 & 0.81 & 2.70  & 7.051$\times$10$^{-4}$ & 0.02 & 2.04 & 441.26 & 0.0 & 6.13 & 257.18 \\ 
20 & 1.19 & 2.28  & 7.000$\times$10$^{-4}$ & 0.02 & 2.63 & 546.35 & 0.0 & 7.9 & 309.65 \\ 
20 & 1.52 & 1.97  & 6.668$\times$10$^{-4}$ & 0.02 & 2.67 & 550.28 & 0.01 & 7.95 & 309.31 \\ 
20 & 1.39 & 1.93  & 6.703$\times$10$^{-4}$ & 0.02 & 2.69 & 553.25 & 0.01 & 7.99 & 311.15 \\ 
20 & 8.86 & 1.74  & 3.555$\times$10$^{-4}$ & 21.11 & 1.41 & 251.2 & 0.04 & 9.19 & 125.35 \\ 
20 & 0.85 & 2.62  & 7.048$\times$10$^{-4}$ & 0.02 & 2.16 & 461.57 & 0.0 & 6.47 & 267.36 \\ 
25 & 1.92 & 3.13  & 1.051$\times$10$^{-4}$ & 1.75 & 0.43 & 96.7 & 0.06 & 2.43 & 46.69 \\ 
25 & 3.07 & 1.83  & 1.051$\times$10$^{-4}$ & 70846.64 & 391.66 & 96.7 & 0.06 & 2.43 & 46.69 \\ 
25 & 3.30 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.43 & 98.54 & 0.06 & 2.36 & 47.64 \\ 
25 & 1.04 & 1.84  & 1.333$\times$10$^{-4}$ & 0.39 & 0.59 & 142.62 & 0.05 & 3.84 & 71.99 \\ 
25 & 9.73 & 2.35  & 1.071$\times$10$^{-4}$ & 13.39 & 0.35 & 82.74 & 0.06 & 1.6 & 43.98 \\ 
25 & 1.20 & 1.84  & 1.333$\times$10$^{-4}$ & 0.39 & 0.62 & 143.1 & 0.05 & 3.84 & 71.99 \\ 
25 & 7.42 & 2.37  & 8.412$\times$10$^{-5}$ & 12.51 & 0.29 & 63.54 & 0.04 & 2.1 & 33.31 \\ 
25 & 18.4 & 2.35  & 1.055$\times$10$^{-4}$ & 22.85 & 0.34 & 78.16 & 0.06 & 2.78 & 42.51 \\ 
25 & 14.8 & 2.35  & 7.676$\times$10$^{-5}$ & 39.45 & 0.22 & 39.56 & 0.07 & 1.87 & 19.07 \\ 
25 & 2.78 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.44 & 98.65 & 0.06 & 2.4 & 47.64 \\ 
25 & 0.89 & 4.66  & 7.431$\times$10$^{-4}$ & 0.11 & 2.07 & 519.83 & 0.0 & 19.64 & 256.34 \\ 
25 & 7.08 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.42 & 98.43 & 0.06 & 2.26 & 47.66 \\ 
25 & 0.92 & 1.84  & 1.333$\times$10$^{-4}$ & 0.39 & 0.63 & 143.21 & 0.05 & 3.84 & 71.99 \\ 
25 & 2.64 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.44 & 98.66 & 0.06 & 2.42 & 47.64 \\ 
25 & 6.17 & 2.38  & 9.114$\times$10$^{-5}$ & 10.03 & 0.33 & 71.51 & 0.04 & 2.12 & 36.85 \\ 
25 & 4.73 & 2.38  & 1.732$\times$10$^{-4}$ & 8.07 & 0.77 & 172.19 & 0.05 & 4.2 & 85.15 \\ 
25 & 1.52 & 1.83  & 1.333$\times$10$^{-4}$ & 0.39 & 0.62 & 143.1 & 0.05 & 3.84 & 71.99 \\ 
25 & 1.57 & 3.73  & 5.518$\times$10$^{-4}$ & 0.54 & 1.93 & 496.11 & 0.03 & 15.48 & 268.45 \\ 
25 & 0.99 & 4.89  & 7.447$\times$10$^{-4}$ & 0.16 & 1.86 & 464.3 & 0.0 & 19.48 & 227.53 \\ 
25 & 8.40 & 2.38  & 1.074$\times$10$^{-4}$ & 14.15 & 0.36 & 83.33 & 0.06 & 2.27 & 44.06 \\ 
25 & 2.53 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.44 & 98.67 & 0.06 & 2.44 & 47.64 \\ 
25 & 4.72 & 2.35  & 1.059$\times$10$^{-4}$ & 1.41 & 0.43 & 98.45 & 0.06 & 2.29 & 47.65 \\ 
\end{tabular}
\label{full_summary_table:continued}
\contcaption{Table of all core collapse model predicted/ESS ratios using $^{26}$Al as the dilution isotope. M$_{prog}$ is the progenitor mass, E$_{exp}$ is the explosion energy, M$_{rem}$ is the remnant mass.}
\end{table*}

==> tables/Summary_data_table_partial.tex <==
\begin{table*}
\centering
\begin{tabular}{rrrr|rrrrrr}
M$_{prog}$& E$_{exp}$& M$_{rem}$& Dilution ($f$) & $^{53}$Mn & $^{60}$Fe & $^{92}$Nb & $^{129}$I & $^{135}$Cs & $^{182}$Hf \\ 
(M$_{\odot})$ & FoE & (M$_{\odot})$ &  &  &  &  &  &  &  \\ 
\hline
15 & 1.90 & 1.62  & 4.134$\times$10$^{-4}$ & 116.6 & 860.61 & 340.01 & 0.93 & 183.94 & 4.02 \\ 
15 & 1.86 & 1.63  & 4.141$\times$10$^{-4}$ & 116.94 & 839.07 & 241.07 & 0.93 & 187.54 & 4.37 \\ 
15 & 1.94 & 1.61  & 4.138$\times$10$^{-4}$ & 117.23 & 877.89 & 286.94 & 0.93 & 182.73 & 3.83 \\ 
15 & 0.54 & 1.91  & 4.45$\times$10$^{-4}$ & 3.12 & 816.91 & 0.05 & 1.09 & 237.88 & 1.54 \\ 
15 & 0.92 & 1.75  & 2.731$\times$10$^{-4}$ & 37.32 & 529.1 & 60.31 & 0.6 & 127.9 & 3.24 \\ 
15 & 1.69 & 1.52  & 3.277$\times$10$^{-4}$ & 97.61 & 700.97 & 3751.67 & 0.74 & 146.96 & 3.02 \\ 
15 & 0.34 & 1.94  & 4.598$\times$10$^{-4}$ & 2.04 & 849.22 & 0.05 & 1.09 & 240.2 & 0.95 \\ 
15 & 3.43 & 1.51  & 2.51$\times$10$^{-4}$ & 64.35 & 1988.7 & 2484.75 & 0.53 & 101.8 & 3.47 \\ 
15 & 2.06 & 1.59  & 4.135$\times$10$^{-4}$ & 124.57 & 913.14 & 1431.69 & 0.93 & 180.34 & 3.46 \\ 
15 & 2.24 & 1.56  & 4.123$\times$10$^{-4}$ & 130.51 & 1009.78 & 5838.45 & 0.92 & 176.86 & 2.86 \\ 
15 & 2.60 & 1.52  & 4.009$\times$10$^{-4}$ & 123.11 & 1364.3 & 7644.28 & 0.89 & 169.71 & 3.67 \\ 
15 & 0.74 & 1.73  & 2.67$\times$10$^{-4}$ & 26.31 & 500.88 & 61.11 & 0.59 & 127.79 & 3.09 \\ 
15 & 0.82 & 1.88  & 4.351$\times$10$^{-4}$ & 22.11 & 803.18 & 0.05 & 1.07 & 234.21 & 3.1 \\ 
15 & 10.7 & 1.53  & 4.126$\times$10$^{-4}$ & 82.12 & 765.06 & 3138.02 & 0.81 & 166.59 & 4.25 \\ 
15 & 2.47 & 1.52  & 3.88$\times$10$^{-4}$ & 98.94 & 866.94 & 211.35 & 0.83 & 160.97 & 2.84 \\ 
15 & 4.79 & 1.50  & 2.472$\times$10$^{-4}$ & 52.46 & 3134.9 & 2879.59 & 0.45 & 89.61 & 3.28 \\ 
15 & 2.63 & 1.53  & 3.412$\times$10$^{-4}$ & 94.63 & 1603.37 & 3770.52 & 0.69 & 133.35 & 4.04 \\ 
20 & 2.85 & 1.74  & 1.684$\times$10$^{-3}$ & 6686.74 & 2283.82 & 0.05 & 7.27 & 1430.95 & 22.39 \\ 
20 & 1.47 & 2.23  & 1.909$\times$10$^{-3}$ & 1056.97 & 2536.84 & 0.0 & 7.32 & 1525.84 & 21.58 \\ 
20 & 2.50 & 1.93  & 8.655$\times$10$^{-4}$ & 38.93 & 1198.62 & 0.02 & 3.89 & 747.01 & 10.41 \\ 
20 & 5.03 & 1.74  & 3.87$\times$10$^{-4}$ & 1425.03 & 615.69 & 55.96 & 1.87 & 360.79 & 12.01 \\ 
20 & 2.76 & 1.76  & 1.412$\times$10$^{-3}$ & 5702.16 & 1925.04 & 0.04 & 6.08 & 1194.49 & 18.49 \\ 
20 & 2.60 & 1.90  & 1.165$\times$10$^{-3}$ & 550.21 & 1607.28 & 0.04 & 5.0 & 981.52 & 15.2 \\ 
20 & 2.43 & 1.86  & 1.649$\times$10$^{-3}$ & 3822.32 & 2234.52 & 0.05 & 6.92 & 1384.3 & 21.49 \\ 
20 & 1.04 & 2.47  & 3.156$\times$10$^{-3}$ & 1675.87 & 3688.55 & 0.0 & 10.63 & 2241.79 & 34.44 \\ 
20 & 4.15 & 1.85  & 3.972$\times$10$^{-4}$ & 1471.01 & 603.48 & 0.13 & 1.98 & 373.16 & 9.49 \\ 
20 & 0.65 & 3.03  & 3.014$\times$10$^{-3}$ & 9.19 & 2464.65 & 0.0 & 6.7 & 1518.29 & 21.76 \\ 
20 & 0.78 & 2.85  & 3.086$\times$10$^{-3}$ & 1096.48 & 2863.47 & 0.0 & 8.0 & 1759.02 & 25.96 \\ 
20 & 0.84 & 2.62  & 3.097$\times$10$^{-3}$ & 1391.11 & 3319.16 & 0.0 & 9.48 & 2027.59 & 30.64 \\ 
20 & 1.00 & 2.35  & 3.093$\times$10$^{-3}$ & 1764.41 & 3855.62 & 0.0 & 11.17 & 2334.12 & 36.02 \\ 
20 & 1.65 & 1.78  & 2.709$\times$10$^{-3}$ & 6462.83 & 3669.31 & 0.04 & 10.86 & 2236.59 & 35.07 \\ 
20 & 0.75 & 2.76  & 3.097$\times$10$^{-3}$ & 1333.48 & 3046.53 & 0.0 & 8.59 & 1868.31 & 27.84 \\ 
20 & 0.53 & 3.40  & 3.014$\times$10$^{-3}$ & 0.16 & 1782.7 & 0.0 & 4.43 & 1107.12 & 14.61 \\ 
20 & 4.33 & 1.87  & 3.803$\times$10$^{-4}$ & 1585.16 & 582.1 & 0.14 & 1.86 & 355.2 & 10.17 \\ 
20 & 0.81 & 2.70  & 3.086$\times$10$^{-3}$ & 1449.62 & 3153.9 & 0.0 & 8.95 & 1930.95 & 28.89 \\ 
20 & 1.19 & 2.28  & 3.133$\times$10$^{-3}$ & 1727.04 & 4051.07 & 0.0 & 11.76 & 2445.8 & 38.07 \\ 
20 & 1.52 & 1.97  & 2.624$\times$10$^{-3}$ & 264.73 & 3552.5 & 0.04 & 10.51 & 2164.98 & 33.88 \\ 
20 & 1.39 & 1.93  & 2.642$\times$10$^{-3}$ & 29.2 & 3577.35 & 0.04 & 10.58 & 2179.85 & 33.97 \\ 
20 & 8.86 & 1.74  & 3.294$\times$10$^{-4}$ & 1460.03 & 1981.15 & 217.44 & 1.34 & 234.95 & 8.41 \\ 
20 & 0.85 & 2.62  & 3.085$\times$10$^{-3}$ & 1446.57 & 3308.32 & 0.0 & 9.44 & 2020.64 & 30.54 \\ 
25 & 1.92 & 3.13  & 7.065$\times$10$^{-5}$ & 470.25 & 455.85 & 0.16 & 0.33 & 67.53 & 1.64 \\ 
25 & 3.07 & 1.83  & 7.065$\times$10$^{-5}$ & 470.29 & 458.63 & 9.58 & 92.06 & 67.53 & 1.64 \\ 
25 & 3.30 & 2.35  & 7.123$\times$10$^{-5}$ & 221.77 & 443.52 & 0.16 & 0.33 & 68.84 & 1.57 \\ 
25 & 1.04 & 1.84  & 9.46$\times$10$^{-5}$ & 407.97 & 460.66 & 14.29 & 0.45 & 103.85 & 2.75 \\ 
25 & 9.73 & 2.35  & 7.223$\times$10$^{-5}$ & 28.6 & 838.73 & 0.17 & 0.27 & 58.42 & 1.06 \\ 
25 & 1.20 & 1.84  & 9.46$\times$10$^{-5}$ & 504.83 & 460.66 & 13.58 & 0.46 & 104.07 & 4.27 \\ 
25 & 7.42 & 2.37  & 5.363$\times$10$^{-5}$ & 282.77 & 702.04 & 0.06 & 0.23 & 44.65 & 1.32 \\ 
25 & 18.4 & 2.35  & 7.088$\times$10$^{-5}$ & 27.61 & 1193.89 & 0.16 & 0.26 & 55.13 & 1.81 \\ 
25 & 14.8 & 2.35  & 5.307$\times$10$^{-5}$ & 276.6 & 1357.57 & 0.22 & 0.19 & 29.01 & 1.26 \\ 
25 & 2.78 & 2.35  & 7.13$\times$10$^{-5}$ & 222.0 & 443.93 & 0.16 & 0.33 & 68.97 & 1.61 \\ 
25 & 0.89 & 4.66  & 1.826$\times$10$^{-3}$ & 0.12 & 6958.27 & 0.0 & 5.08 & 1276.89 & 51.22 \\ 
25 & 7.08 & 2.35  & 7.126$\times$10$^{-5}$ & 221.86 & 443.72 & 0.16 & 0.32 & 68.78 & 1.5 \\ 
25 & 0.92 & 1.84  & 9.46$\times$10$^{-5}$ & 504.84 & 460.66 & 13.58 & 0.46 & 104.11 & 3.08 \\ 
25 & 2.64 & 2.35  & 7.13$\times$10$^{-5}$ & 222.0 & 443.93 & 0.16 & 0.33 & 68.98 & 1.62 \\ 
25 & 6.17 & 2.38  & 5.847$\times$10$^{-5}$ & 304.41 & 650.31 & 0.06 & 0.25 & 50.22 & 1.34 \\ 
25 & 4.73 & 2.38  & 1.363$\times$10$^{-4}$ & 527.44 & 1020.98 & 0.67 & 0.61 & 138.39 & 3.24 \\ 
25 & 1.52 & 1.83  & 9.46$\times$10$^{-5}$ & 505.92 & 460.66 & 5.19 & 0.46 & 104.06 & 5.6 \\ 
25 & 1.57 & 3.73  & 9.342$\times$10$^{-4}$ & 0.09 & 4110.9 & 0.0 & 3.19 & 842.15 & 26.14 \\ 
25 & 0.99 & 4.89  & 1.823$\times$10$^{-3}$ & 0.11 & 6923.3 & 0.0 & 4.56 & 1136.17 & 47.94 \\ 
25 & 8.40 & 2.38  & 7.23$\times$10$^{-5}$ & 11.86 & 868.0 & 0.17 & 0.28 & 58.75 & 1.5 \\ 
25 & 2.53 & 2.35  & 7.13$\times$10$^{-5}$ & 222.01 & 443.93 & 0.16 & 0.33 & 68.98 & 1.64 \\ 
25 & 4.72 & 2.35  & 7.118$\times$10$^{-5}$ & 221.59 & 443.17 & 0.16 & 0.33 & 68.72 & 1.52 \\ 
\end{tabular}
\caption{Table of isotopes core collapse model predicted/ESS ratios using $^{26}$Al as the dilution isotope. M$_{prog}$ is the progenitor mass, E$_{exp}$ is the explosion energy, M$_{rem}$ is the remnant mass. A full table can be found XXX}
\end{table*}

==> tables/ess_latex_form.tex <==
\begin{table*}
\centering
\begin{tabular}{c|ccccc}
\hline
SLR & Daughter & Reference & T$_{1/2}$ (yr) & $\tau$ (yr) & ESS ratio \\ 
\hline
$^{10}$Be & $^{10}$B & $^{9}$Be & 1.388$\times$10$^{6}$ & 2.002$\times$10$^{6}$ & (6$\pm$3)$\times$10$^{-4}$  \\ 
$^{26}$Al & $^{26}$Mg & $^{27}$Al & 7.170$\times$10$^{5}$ & 1.034$\times$10$^{6}$ & (5.23$\pm$0.13)$\times$10$^{-5}$  \\ 
$^{36}$Cl & $^{36}$S & $^{35}$Cl & 3.010$\times$10$^{5}$ & 4.343$\times$10$^{5}$ & (2.44$\pm$0.65)$\times$10$^{-5}$  \\ 
$^{41}$Ca & $^{41}$K & $^{40}$Ca & 9.940$\times$10$^{4}$ & 1.434$\times$10$^{5}$ & (4.6$\pm$1.9)$\times$10$^{-9}$  \\ 
$^{53}$Mn & $^{53}$Cr & $^{55}$Mn & 3.740$\times$10$^{6}$ & 5.396$\times$10$^{6}$ & (7$\pm$1)$\times$10$^{-6}$  \\ 
$^{60}$Fe & $^{60}$Ni & $^{56}$Fe & 2.620$\times$10$^{6}$ & 3.780$\times$10$^{6}$ & (1.01$\pm$0.27)$\times$10$^{-8}$  \\ 
$^{92}$Nb & $^{92}$Zr & $^{92}$Mo & 3.470$\times$10$^{7}$ & 5.006$\times$10$^{7}$ & (3.2$\pm$0.3)$\times$10$^{-5}$  \\ 
$^{97}$Tc & $^{97}$Mo & $^{98}$Ru & 4.210$\times$10$^{6}$ & 6.074$\times$10$^{6}$ & <1.1$\times$10$^{-5}$  \\ 
$^{98}$Tc & $^{98}$Ru & $^{98}$Ru & 4.200$\times$10$^{6}$ & 6.059$\times$10$^{6}$ & <6$\times$10$^{-5}$  \\ 
$^{107}$Pd & $^{107}$Ag & $^{108}$Pd & 6.500$\times$10$^{6}$ & 9.378$\times$10$^{6}$ & (6.6$\pm$0.4)$\times$10$^{-5}$  \\ 
$^{126}$Sn & $^{126}$Te & $^{124}$Sn & 2.300$\times$10$^{5}$ & 3.318$\times$10$^{5}$ & <3$\times$10$^{-6}$  \\ 
$^{129}$I & $^{129}$Xe & $^{127}$I & 1.570$\times$10$^{7}$ & 2.265$\times$10$^{7}$ & (1.28$\pm$0.03)$\times$10$^{-4}$  \\ 
$^{135}$Cs & $^{135}$Ba & $^{133}$Cs & 2.300$\times$10$^{6}$ & 3.318$\times$10$^{6}$ & <2.8$\times$10$^{-6}$  \\ 
$^{146}$Sm & $^{142}$Nd & $^{144}$Sm & 6.800$\times$10$^{7}$ & 9.810$\times$10$^{7}$ & (8.28$\pm$0.44)$\times$10$^{-3}$  \\ 
$^{182}$Hf & $^{182}$W & $^{180}$Hf & 8.900$\times$10$^{6}$ & 1.284$\times$10$^{7}$ & (1.018$\pm$0.043)$\times$10$^{-4}$  \\ 
$^{205}$Pb & $^{205}$Tl & $^{204}$Pb & 1.730$\times$10$^{7}$ & 2.496$\times$10$^{7}$ & (1.8$\pm$1.2)$\times$10$^{-3}$  \\ 
\end{tabular}
\label{tab:ess_ref_table}
\caption{All SLRs listed with reference isotopes, T$_{1/2}$, $\tau$, and ESS ratios. Data gathered from \cite{Lugaro2018}. If no error is given this value is an upper limit. We do not consider $^{10}$Be in this work due to not being produced significantly in supernovae. \textcolor{red}{Fix the sig. figs, choose between half lives, }}
\end{table*}

==> tables/h_ing_correction_table.tex <==
\begin{table}
\centering
\label{tab:h_ing_correction_table}
\begin{tabular}{c|c}
Isotope & Correction Factor \\ 
\hline
AL 27 & 1.463$\times$10$^{0}$ \\ 
AL 26 & 1.408$\times$10$^{1}$ \\ 
FE 60 & 1.261$\times$10$^{-2}$ \\ 
\end{tabular}
\caption{Correction factors applied to the models in order to replicated hydrogen ingestion. These factors are applied to the relevant isotopes before any dilution of time delay factors are applied. Details can be found in \cite{Pignatari2016a}}
\end{table}
